Termination and Confluence of Higher-Order Rewrite Systems

In the last twenty years, several approaches to higher-order rewriting have been proposed, among which Klop's Combinatory Rewrite Systems (CRSs), Nipkow's Higher-order Rewrite Systems (HRSs) and Jouannaud and Okada's higher-order algebraic specification languages, of which only the last one considers typed terms. The later approach has been extended by Jouannaud, Okada and the present author into Inductive Data Type Systems (IDTSs). In this paper, we extend IDTSs with the CRS higher-order pattern-matching mechanism, resulting in simply-typed CRSs. Then, we show how the termination criterion developed for IDTSs with first-order pattern-matching, called the General Schema, can be extended so as to prove the strong normalization of IDTSs with higher-order pattern-matching. Next, we compare the unified approach with HRSs. We first prove that the extended General Schema can also be applied to HRSs. Second, we show how Nipkow's higher-order critical pair analysis technique for proving local confluence can be applied to IDTSs.

==> eta.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% about eta
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the definition given in \cite{}, the rewrite relation which was
considered was the union $\a_\b \cup \a_\e \cup \a_\cR$. Now, the rule
$\b$ is not seen as a special rule: it is part of $\cR$. But, what can
we say about $\e$ ? Since rule left-hand sides must be headed by
function symbols, it is not possible to consider the rule

\begin{center}
$[x]@(Z,x) \a Z$
\end{center}

On the other hand, it is always possible to extend the alphabet with
symbols $\l_{s,t} \in F_{s\a t, s\a t}$, and restrict the set of terms
to the terms whose subterms of the form $[x]u$ are always headed by
some $\l_{s,t}$. Such a set is clearly stable by reduction.
Furthermore, since the type indices $s,t$ may be recovered by doing a
type analysis, they may be dropped. Hence, by writting
$\l_{s,t}([x]u)$ simply $\l x.u$, we recover a more usual syntax and
the rule

\begin{center}
$\l x.@(Z,x) \a Z$
\end{center}

\noindent
may be part of $\cR$. Thus, it is possible to include $\e$ in $\cR$,
if one restricts oneself to the set of terms described above.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lambda-extension
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A second kind of IDTS will also interest us, but rather for applying
Nipkow's higher-order critical pair technique for proving local
confluence in Section~\ref{}.

\begin{dfn}[$\l$-extension]
The {\em $\l$-extension} of an IDTS-alphabet $\cA = (\cB, \cX, \cF,
\cZ)$ is the IDTS-alphabet $\l\cA = (\cB, \cX, \cF', \cZ)$ where:
\begin{lst}{--}
\item $F'_{s_1, \ldots, s_n,s} = F_{s_1, \ldots, s_n,s}$ if $n \neq 1$
  or else $s_1 = s = t_1 \a t_2$,
\item $F'_{s\a t, s\a t} = F_{s\a t, s\a t} \cup \{ \l_{s,t} \}$.
\end{lst}

\noindent
Then, the set $\l\cI(\cA)$ of {\em $\l\cI(\cA)$-terms} is the subset
of $\cI(\cA)$-terms whose subterms of the form $[x]u$ are always
headed by some $\l_{s,t}$. Given a $\cI(\cA)$-term $u$, we denote by
$u^\l$ the $\l\cI(\cA)$-term obtained by adding $\l_{s,t}$ above each
subterm of $u$ of the form $[x]v$.

\noindent
The {\em $l$-extension} of an IDTS $\cI = (\cA, \cR)$ is the IDTS
$\l\cI = (\l\cA, \l\cR)$ where $\l\cR = \{ l^\l \a r^\l ~|~ l\a r \in
\cR \}$. Finally, we say that an IDTS is a {\em $\l$-IDTS} if it is
the $\l$-extension of some IDTS.
\end{dfn}

Since $\l\cI(\cA)$ is stable by reduction, $\l$-extensions enjoys the
following properties:

\begin{lem}
  $\cI$ is strongly normalizing (resp. confluent, locally confluent)
  iff $\l\cI$ is strongly normalizing (resp. confluent, locally
  confluent) on $\l\cI$-terms.
\end{lem}

As in the case of $@$, it is possible to drop the type indices. And
since, in a $\l\cI$-term, every subterm of the form $[x]u$ is headed
by some $\l_{s,t}$, it is possible to write it $\l x. u$. By this way,
the syntax of $\cI$ and $\l\cI$ are quite similar: $[x]u$ is merely
replaced by $\l x.u$.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

